Decentralized Graph Neural Network for Privacy-Preserving Recommendation

Building a graph neural network (GNN)-based recommender system without violating user privacy proves challenging. Existing methods can be divided into federated GNNs and decentralized GNNs. But both methods have undesirable effects, i.e., low communication efficiency and privacy leakage. This paper proposes DGREC, a novel decentralized GNN for privacy-preserving recommendations, where users can choose to publicize their interactions. It includes three stages, i.e., graph construction, local gradient calculation, and global gradient passing. The first stage builds a local inner-item hypergraph for each user and a global inter-user graph. The second stage models user preference and calculates gradients on each local device. The third stage designs a local differential privacy mechanism named secure gradient-sharing, which proves strong privacy-preserving of users' private data. We conduct extensive experiments on three public datasets to validate the consistent superiority of our framework.

==> checklist.tex <==
\section*{Checklist}
\begin{enumerate}
\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See Section~\ref{section_method} and \ref{section_experiment}.}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{subsec_performance_comparison} and \ref{section_conclusion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{Our work aims to solve one of the negative societal impacts from recommender systems, i.e., violating user privacy.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
\item Did you state the full set of assumptions of all theoretical results?
\answerYes{See Theorems \ref{theorem_gradient_encoding_rdp}, \ref{theorem_gradient_encoding_privacy_budget} and Propositions \ref{proposition_gradient_encoder}, \ref{proposition_convergence}.}
\item Did you include complete proofs of all theoretical results?
\answerYes{See Section \ref{appendix_proof_theorem1}, \ref{appendix_gradient_encoder_budget} and \ref{appendix_gradient_encoder}.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See code and instructions in the supplemental material and we cite the data source in \ref{subsec_experiment_settings}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section \ref{subsec_experiment_settings}.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See Section \ref{subsec_performance_comparison}.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{The consumed resources vary with the methods and hyperparameters, but we can launch all experiments on a single NVIDIA GeForce RTX 3090.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See Section \ref{subsec_experiment_settings}}
  \item Did you mention the license of the assets?
    \answerYes{They are public datasets.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{See Section \ref{subsec_experiment_settings}}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{See Section \ref{subsec_experiment_settings}}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> discussion_and_future_work.tex <==
\section{Discussion and future work}
%
This paper mainly aims to provide a privacy-preserving recommendation framework, which highlights superior recommendation performance and strong privacy protection.
%
Under the strict data protection regulations, such as GDPR\footnote{https://gdpr-info.eu}, online platforms and giant enterprises are no longer able to collect user private data and then make correct recommendations.
%
However, we still need recommender systems to alleviate the information overload problem.
%
The privacy-preserving recommender system with high performance is worth studying, and we hope more researchers will join in this field.

%
In future work, we plan to address the limitations of our work.
%
We will extend our research to untrusted environments where other clients may be semi-honest and malicious, and study cryptography techniques to solve the issue, e.g., zero-knowledge proof.
%
Meanwhile, we will further investigate defense methods against poisoning attacks.

==> main_reason_for_rejection.tex <==
\section{Main reason for rejection}
%
Our paper received three reviews, including a `Reject' (3), an `Accept' (7), and an `Accept' (7). 
%
The average rating of our paper is 5.67.
%
Unfortunately, we got reject at the final decision.
%
We list the main concerns of the first reviewer as follows.
%
(1) The motivation of the method design is not clear.
%
(2) The assumption in the paper are rather too strong.
%

\section{Main changes and improvements}
%
We have solved all the concerns raised by the reviewers.
%
We list the main changes and improvements as follows.

%
\nosection{Detailed motivations of the method design} 
We have added the motivations at the beginning of each method in our main paper, and summarize the motivations of each method in Appendix~\ref{detailed_overview_of_techniques}.
%
To further elaborate the concepts, we have provided detailed related work about GNN and privacy-preserving methods in Appendix~\ref{Related_work_in_details}.
%
% We have also provided a detailed overview of the used techniques in Section~\ref{detailed_overview_of_techniques}.

\nosection{More supports for our assumption}
%
In introduction \textbf{CH1}, we have added examples in real world to demonstrate that users are willing to publish part of their interactions, and taking all interactions as private causes setbacks in user experience.
%
In building graphs, we have made it more clear that the user graph is constructed through communication protocols, other than being stored in a user's device.
%
We have also added reference to support that our system is practical.
%
% In neighbor sampling (Section~\ref{subsection_global_gradient_passing}), we have revised our expression, avoiding misunderstanding for assumptions.

%
\nosection{More technical details} Instead of proving that our secure gradient sharing can protect each element of the gradient, we have further proved its ability to protect the whole gradient in Appendix~\ref{appendix_proof_theorem1}.
%
Besides, we have theoretically proved that our method has the lowest communication cost among all competitors in Appendix~\ref{subsection_communication_cost}.

==> overview_of_used_techniques.tex <==
\section{An overview of motivations}
\label{detailed_overview_of_techniques}
%
In this section, we provide a detailed overview of the motivations for each method as follows.

\nosection{Motivations behind a user graph}
%
A graph structure is expressive to represent non-Euclidean data, e.g., social relationships.
%
Here, we construct a normal user graph, where nodes are the users, and edges are originated from user friendship or proximity.
%
The constructed user graph supports the downstream neighbor sampling and secure gradient sharing.

%
\nosection{Motivations behind an item hypergraph}
We are only allowed to model user preference from his interacted items as well as neighbors' public items, given that most interactions are private.
%
To stabilize model training, we leverage item categories (tags) to build the graph, avoiding calculating item relationships for each training step.
%
Since an item generally has several tags, and tag information is not related to our main task, we construct an item hypergraph, instead of modeling item-tag relationships explicitly.
%
% In an item hypergraph, nodes are the items, and hyper

\nosection{Motivation behind graph distillation}
%
In the constructed hypergraph, connected items tend to reflect similar user preferences, since they have the same tags or categories.
%
But user interests are dispersed.
%
To build a concrete interest graph, we leverage hypergraph convolution networks to distill the constructed hypergraph.

%
\nosection{Motivation behind pearson loss}
Since the distilled interest can be correlated and even redundant, we leverage Pearson loss to encourage the distilled interests to be independent.

\nosection{Motivation behind interest pooling}
%
Given that noisy behaviors commonly exist in user interactions, and neighboring users do not constantly share the same interests, we propose interest attention mechanism under GNN architecture, to minimize the weight of noisy interests.

\nosection{Motivation behind neighbor sampling}
%
Two problems remain unresolved in model training, which damage model performance.
%
(1) Some items are not fully trained, or even not trained, since user-item interactions are sparse in recommendation scenarios.
%
(2) Different users have different convergence speeds.
%
Based on the global user graph, we design a sampling strategy to involve more users in model training, where underfit user models are more likely to be sampled.

\nosection{Motivation behind gradient encoding}
To secure gradient sharing and minimize communication cost, we propose gradient encoding to encode each element of the gradients into 1-bit.

\nosection{Motivation behind gradient propagation}
%
In our setting, user can only communicate with his own neighbors. 
%
Motivated by message passing mechanisms in GNNs, where node features are passed within neighbors, we propose gradient propagation that each user in the neighborhood sends and receives gradients from his neighbors.

\nosection{Motivation behind gradient decoding}
%
Conventional LDP mechanisms protect user privacy at the cost of introducing noises to model training, which degrades training convergence.
%
We propose gradient decoding to decode all received gradients in a noise-free way.

==> proof.tex <==
\section{Proof}
\subsection{Proof of Theorem 1}
\label{appendix_proof_theorem1}
\begin{proof}
%
Let $\mathcal{M}(g)$ be the secure gradient sharing as described in Equation (5).
%
We need to show that for any two input gradients $g$ and $g^{\prime}$, we have $D_{\alpha}(M(g)\parallel M(g^{\prime})) \le \epsilon$.
%
For the $i$-th element of the encoded gradient, $g_{i}^{*} \in \{-1, 1\}$.
%
We let $z=e^{\beta}+1$ to simplify the description.
%
Then, for two continuous distributions, P and Q, defined over the real interval with densities $p$ and $q$, we have
%
\begin{equation}
\begin{aligned}
    p(g) &= \mathrm{P}[\mathcal{M}(g)=1] = \frac{\delta z + (z-2)g}{2\delta z}, \\
    q(g) &= \mathrm{P}[\mathcal{M}(g)=-1] = \frac{\delta z - (z-2)g}{2\delta z}. \nonumber
\end{aligned}
\end{equation}
%
Given that we clip gradients $g$ into $\left[-\delta, \delta \right]$, we can evaluate $D_{\alpha}(M(g)\parallel M(g^{\prime}))$ separately over three intervals, i.e., $\left(-\infty, -\delta \right)$, $\left[-\delta, \delta \right]$, and $\left(\delta, +\infty \right)$.
%
Here, we let $n_{s}$ denote the size of the gradient.
%
Then, we have,
%
\begin{equation}
\begin{aligned}
D_{\alpha}(M(g)\parallel M(g^{\prime})) &= \frac{1}{\alpha - 1}log \prod \limits_{i=0}^{ns} \int_{-\infty}^{\infty}p(g_{i})^{\alpha}q(g_{i})^{1-\alpha}\mathrm{d} g_{i}\\
&= \frac{1}{\alpha - 1} \sum \limits_{i=0}^{ns} log\int_{-\infty}^{\infty} p(g_{i})^{\alpha}q(g_{i})^{1-\alpha}\mathrm{d} g_{i}.\nonumber
\end{aligned}
\end{equation}
%
For intervals $\left(-\infty, -\delta \right)$ and $\left(\delta, +\infty \right)$, we have
%
\begin{equation}
\begin{aligned}
\int_{-\infty}^{-\delta}p(g)^{\alpha}q(g)^{1-\alpha}\dif g &= \frac{(z-1)^{1-\alpha}}{z},\\
\int_{\delta}^{\infty}p(g)^{\alpha}q(g)^{1-\alpha}\dif g &= \frac{(z-1)^{\alpha}}{z} \nonumber.
\end{aligned}
\end{equation}
%
For intervals $\left[-\delta, \delta \right]$,
we let $x=(z-2)g$ and $y=\delta z$. 
%
Then we have
\begin{small}
\begin{equation}
\begin{aligned}
\int_{-\delta}^{\delta}p(g)^{\alpha}q(g)^{1-\alpha}\dif g &= \frac{1}{2\delta z(z-2)}\int_{-y + 2\delta}^{y - 2\delta}(x+y)^{\alpha}(-x+y)^{1-\alpha} \dif x  \\
&\le \frac{1}{2\delta z(z-2)}\int_{-y}^{y}(x+y)^{\alpha}(-x+y)^{1-\alpha} \dif x \nonumber.
\end{aligned}
\end{equation}
\end{small}
Given the reverse chain rule, we let $t=(x+y)/2y$ and have 
%
\begin{equation}
\begin{aligned}
\int_{-\delta}^{\delta}p(g)^{\alpha}q(g)^{1-\alpha}\dif g &= \frac{1}{z-2}\int_{0}^{1}(2yt)^{\alpha}(-2yt+2y)^{1-\alpha} \dif t \\
&= \frac{2\delta z}{z-2}\int_{0}^{1}(t)^{\alpha}(-t+1)^{1-\alpha} \dif t \nonumber.
\end{aligned}
\end{equation}
According to the definition of beta and gamma functions, we have
\begin{equation}
\begin{aligned}
\int_{-\delta}^{\delta}p(g)^{\alpha}q(g)^{1-\alpha}\dif g &= \frac{2\delta z}{z-2}\mathcal{B}(\alpha+1, 2-\alpha) \\
&= \frac{2\delta z}{z-2}\frac{\Gamma(\alpha+1)\Gamma(2-\alpha)}{\Gamma(3)} \\
&= \frac{2\delta z\alpha(\alpha-1)}{(z-2)}\frac{\Gamma(\alpha-1)\Gamma(1-(\alpha-1 ))}{\Gamma(3)} \nonumber.
\end{aligned}
\end{equation}
Then by the reflection formula for the gamma function, we have 
\begin{equation}
\begin{aligned}
\int_{-\delta}^{\delta}p(g)^{\alpha}q(g)^{1-\alpha}\dif g &= \frac{2\delta z\alpha(\alpha-1)\pi}{(z-2)\Gamma(3)sin((\alpha-1) \pi)}\nonumber.
\end{aligned}
\end{equation}
To calculate $D_{\alpha}(M(g)\parallel M(g^{\prime}))$, here we set $\alpha = 1.5$.
%
Then, we have
\begin{small}
\begin{equation}
\begin{aligned}
D_{\alpha}(M(g)\parallel M(g^{\prime})) = 2n_{s}log(\frac{1.5\pi \delta (e^{\beta} + 1)}{2(e^{\beta} - 1)} + \frac{e^{-0.5\beta} + e^{1.5\beta}}{e^{\beta} + 1}) \le \epsilon \nonumber,
\end{aligned}
\end{equation}
\end{small}
%
which concludes the proof of $(1.5, \epsilon)$-RDP.
\end{proof}

\subsection{Proof of Theorem 2}
\label{appendix_gradient_encoder_budget}
\begin{proof}
%
We need to verify that the privacy budget is bounded.
%
We have proved that the secure gradient sharing satisfies $(1.5, \epsilon)$-RDP for one training iteration.
%
Given $T$ training iterations, the secure gradient sharing satisfies $(1.5, \epsilon T)$-RDP, according to the sequential composition~\cite{sequential_composition}.
%
The key property of RDP~\cite{renyi_differential_privacy} is that if $\mathcal{M}(g)$ satisfies $(\alpha, \epsilon)$-RDP, then $\forall \gamma > 0$, $\mathcal{M}(g)$ satisfies $(\epsilon^{\prime}, \gamma)$-DP for $\epsilon^{\prime} = \epsilon + \frac{log(1/\gamma)}{\alpha-1}$. 
%
Then, we conclude that the secure gradient sharing mechanism satisfies $(\epsilon T+2log(1/\gamma ), \gamma)$-DP.
%
We can further choose large $\gamma$ to reduce the privacy budget, which concludes that the privacy budget is bounded.
\end{proof}


\subsection{Proof of Proposition 1}
\label{appendix_gradient_encoder}
\begin{proof}
%
To prove the secure gradient sharing mechanism is noise-free, we need to verify that $E(\bar{g}) = E(g)$.
%
Since the gradients are encoded from the Bernoulli distribution in Equation (5), we have
%
\begin{equation}
\begin{aligned}
    E(g^{*}) =\frac{e^\beta-1}{e^\beta+1}\frac{E(g) + \delta}{\delta} -\frac{e^\beta-1}{e^\beta+1}
    = \frac{(e^\beta-1)E(g)}{(e^\beta+1)\delta} \nonumber.
\end{aligned}
\end{equation}
%
Combining Equation (6), we then have 
\begin{equation}
\begin{aligned}
    E(\bar{g}) &= \frac{\delta(e^\beta + 1)}{e^\beta - 1}E(g^{*}) \\
    &= \frac{\delta(e^\beta + 1)}{e^\beta - 1}\frac{(e^\beta-1)E(g)}{(e^\beta+1)\delta} \\
    &= E(g) \nonumber.
\end{aligned}
\end{equation}
It concludes that the secure gradient-sharing mechanism is noise-free.
\end{proof}


